Database-Backed Web Applications in the Wild: How Well Do They Work?

Most modern database-backed web applications are built upon Object Relational Mapping (ORM) frameworks. While ORM frameworks ease application development by abstracting persistent data as objects, such convenience often comes with a performance cost. In this paper, we present CADO, a tool that analyzes the application logic and its interaction with databases using the Ruby on Rails ORM framework. CADO includes a static program analyzer, a profiler and a synthetic data generator to extract and understand application's performance characteristics. We used CADO to analyze the performance problems of 27 real-world open-source Rails applications, covering domains such as online forums, e-commerce, project management, blogs, etc. Based on the results, we uncovered a number of issues that lead to sub-optimal application performance, ranging from issuing queries, how result sets are used, and physical design. We suggest possible remedies for each issue, and highlight new research opportunities that arise from them.

==> Makefile <==
PAPER_NAME=main
CAMERA_NAME=$(PAPER_NAME)
# Halt on errors instead of going to the shell
LATEX_OPTS=-halt-on-error -mode=batch

default: paper

figs:
	make -C figures/

#fast: figs Makefile
fast:
	pdflatex $(LATEX_OPTS) $(PAPER_NAME)

#paper: figs Makefile
paper:
	pdflatex $(LATEX_OPTS) $(PAPER_NAME)
	bibtex -min-crossrefs=30000 $(PAPER_NAME)
	pdflatex $(LATEX_OPTS) $(PAPER_NAME)
	pdflatex $(LATEX_OPTS) $(PAPER_NAME)
	pdflatex $(LATEX_OPTS) $(PAPER_NAME)
	ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.4 -dEmbedAllFonts=true -dSubsetFonts=true -r600 $(PAPER_NAME).pdf $(PAPER_NAME)_opt.pdf
	mv $(PAPER_NAME)_opt.pdf $(PAPER_NAME).pdf

tidy: Makefile
	rubber --clean $(PAPER_NAME)
	rm -f auto_header.tex

warn: paper
	pdflatex $(PAPER_NAME).tex 2>&1 | grep Warning
	#rubber -W all $(PAPER_NAME).tex

clean: tidy
#	make -C figures/ clean
	rm -f $(PAPER_NAME).pdf rubber.cache

ASPELL_CMDS=\
        --add-tex-command="autoref p" \
        --add-tex-command='bibliography p' \
        --add-tex-command='bibliographystyle p' \
        --add-tex-command='cc p' \
        --add-tex-command='mathrm p' \
        --add-tex-command='newcommand pp' \
        --add-tex-command='renewcommand pp' \

spell:
	@ for i in *.tex; do aspell -t $(ASPELL_CMDS) -p ./aspell.words -c $$i; done
	@ ( head -1 aspell.words ; tail -n +2 aspell.words | sort ) > aspell.words~
	@ mv aspell.words~ aspell.words


==> multiple_queries.tex <==
\section{Interaction among queries}
In this section, we look into the interaction among queries. 
More specifically, we study how caching and prefetching can help 
improve performance. 

For caching, we present our findings on caching intermediate
query results within action to accelerate queries 
with partially matched predicates.
We also examine the caching across actions, mainly the
optimistic performance improvement by general caching, and caching for
synthetically-equivalent queries.

For prefetching, we study the optimistic improvement
by prefetching, and discuss how can the AFG constructed by \tool
help design prefetching scheme.

\subsection{Caching}
We study the opportunity for both intra-action
and inter-action caching. Within an action, Rails already caches the 
results for each query and serve later queries
if the query string is identical. Across actions, Rails by default 
discard all query results unless the developer explicitly implements
cache. With intra-action analysis, we study the benefit of caching 
intermediate query results to server synthetically non-equivalent queries.
For caching across actions, we study the optimistic performance gain
of caching: the percentage of queries whose results can be found in the data
returned by previous queries. We also check the performance gain of a simple
cache that store the query results and hit by matching the query string. 

\paragraph{Intra-action caching}
For queries within an action, we study the opportunities to use cache
 when queries are not synthetically equivalent. To be more specific,
we look into how to cache the intermediate query results
to accelerate later queries when the query predicates partially match.

Since in Rails all queries are generated by ORM from object-oriented language,
we are able to analyze the program, instead of query log, to find out the shared 
query predicate. 
In the program, some predicates are usually stored in 
a program variable, which is used later to issue different queries.
An example is shown in~\listref{queryIntermediate}.
First the {\tt messages} variable is created on line~\lstref{messageSelect} to store
predicates {\tt author\_id=1}.
After that the {\tt any?} function on~\lstref{messageAny} issues a {\tt COUNT} query.
Then messages are later rendered with their author and receipient information 
(~\lstref{messageInclude}), issueing a {\tt JOIN} query.
 The {\tt JOIN} query on~\lstref{messageJoin} partially shares
select condition ({\tt messages.author\_id=1}) 
with the {\tt COUNT} query on~\lstref{messageCount}.

\cong{I may need another example since COUNT can be calculated from index.}
\begin{lstlisting}[language=Ruby,caption={Code snippet from lobsters, 
example of queries partially share predicate},label={queryIntermediate}]
messages = Message.where(:author_id = 1)  @\lstlabel{messageSelect}@
if messages.any? @\lstlabel{messageAny}@
	messages.includes(:author, :recipient).each do |msg|
		render(msg, msg.author, msg.recipient)
	end
end
\end{lstlisting}

\begin{lstlisting}[language=SQL, caption={Corresponding SQL queries issued by Listing X},label={SQLqueryIntermediate}]
SELECT COUNT(*) FROM messages where author_id = 1 @\lstlabel{messageCount}@
SELECT messages.*, User.* FROM messages INNER JOIN users WHERE messages.author_id = User.id OR messages.recipient_id = User.id @\lstlabel{messageJoin}@
\end{lstlisting}

\cong{Evaluation in profiling TBD. }

For each application, we analyze the code to find out how many queries are issued
by the same program variable, which indicates the number of queries that share some
predicates with other queries. The result is shown in~\figref{queryPartial}.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/general_queryPartial.pdf}
  \caption{Queries partially share predicates with other queries}
  \figlabel{queryPartial}
\vspace{-0.1in}
\end{figure}

\begin{mybox}
\textbf{Observation}: 16\% of the queries partially share predicates with other queries.

\textbf{Optimization}: Caching intermediate query results involving the partially shared
predicates can accelerate these queries, and program analysis can identify these queries
and their shared predicates.
\end{mybox} 

\paragraph{Inter-action caching}
By default Rails clear the query cache after an action finishes, 
so no data is shared across actions.
However, query results of a current action can be reused to serve queries in later actions. 
so we analyze the chance of performance improvement by caching queries across actions.

For the inter-action analysis, we focus on caching opportunities within a user session.
We simulate a user session by randomly visiting 9 pages\footnote{\small{We choose 9 
to be the number of pages per user session (not including the login page)
since the average number of visits per day per user for the 10 most popular website in
the U.S. is 8.35~\cite{alexa}.}}, and study the caching opportunities within a user session.

We first calculate the optimistic performance gain by caching. 
For each query, we check whether all the results can be found in the data retrieved by 
all previous queries in the session. 
If yes, this query can be executed using cached data without fetching
any data from the database ('hit' query). 

Then we check that for each query, whether a synthetically-equivalent 
query has been executed before in the same session.
If yes, the query's result can be easily retrieved from cache by 
matching query string (assuming the cache content is correctly updated). Within 
these queries, we also counted how many queries return different results
from previous synthetically-equivalent queries. This difference is due to
writes to the database. The frequency of such queries, synthetically-equivalent
but with different results, reflects the cache update frequency.  

%In above the 'same query' refers to the queries synthetically equivalent, but may return
%different results due to the writes to the database. So we check within the 'same' query
%category, how many queries return different results comparing to the cached synthetically-equivalent
%queris. 
%\cong{Cache update stats TBD.}
%mention that simulating user behavior, short sequence.

%The 'same' and 'same updated' queries can be identified by program analysis. 
%Since the static analysis is unable to know the parameters, it can only point out
%queries with the same template ignoring parameters, which is a super set of 'same' and 'same updated'
%queries. The result of static analysis is shown in~\figref{xxx}.

\cong{static analysis results TBD.}

We measure the queries using both the number of queries and query running time. 
The results are shown in~\figref{cachingQNumber} and~\figref{cachingQTime}.
For all applications profiled, in average 60\% of the read queries
can be read from cache, and 43\% are the same query. In terms of
query running time, the percentage is much smaller: 23.6\% for hit queries
and 17.6\% for synthetically-equivalent queries. 
For cache update frequency,
xx\% of the synthetically-equivalent queries return different results.

There are two main reasons behind the significant percentage of 
synthetically-equivalent queries: 1) Rails support filters for classes, and the
code fragment in the filters are executed everytime a class member function
is called. If different actions calls any function in the same class,
the same code is executed and queries issued in the code are the same;
2) Same layouts are shared by many pages, thus same queries are
issued when generating these layouts.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/cachingQNumber.pdf}
  \caption{Two breakdowns of read queries in terms of query number. Calculated
from profiling results.}
  \figlabel{cachingQNumber}
\vspace{-0.1in}
\end{figure}

\cong{Also point out program analysis can help identify caching candidate.}

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/cachingQTime.pdf}
  \caption{Two breakdowns of read queries in terms of query running time. Calculated
from profiling results.}
  \figlabel{cachingQTime}
\vspace{-0.1in}
\end{figure}


\begin{mybox}
\textbf{Observation}: In one user session, 60\% of queries can be read from cache 
if queries are perfectly cached (which counts for 23.6\% in query running time), 
46\% of the queries are executed previously (17.6\% in running time). 

\textbf{Optimization}:  
\end{mybox}

However, since only 23.6\% of query time can be saved if a perfect cache is 
designed for user session, developers need to consider prefetching query results
in order to further shorten the response time.

\subsection{Prefetching}

In this section we study the potential performance gain of prefetching. As mentioned in~\secref{xxx},
when a user is on current webpage, she can send another request to the server by either
clicking a link on the current page, or filling and submitting a form. In the former case,
the parameters to the next action is given in the url, thus such action
can be pre-run and queries in the action can be prefetched. In the latter case,
the parameters comes from the unpredictable content that user fills in the form, 
and the queries using the user input in the next action cannot be prefetched. 

In the profiling, we treat the queries in the next action triggered by a 'GET' http request as
prefetchable, while queries triggered by a 'POST' request and uses user input (parameters in the 'POST'
request) as non-prefetchable. Intuitively, often more urls 
are listed on a single page than the forms to be filled, 
so most queries do not take random user input and can be prefetchable. This is confirmed by the 
results in~\figref{cacheQNumber} and~\figref{cacheQTime}, 
which show that most queries (93.6\% in number and 98.7\% in time) are prefetchable.

%In~\secref{xxx} we explained how we build AFG, which includes the connection between actions.
%The program analysis can identify the next actions triggered by clicking links or submitting forms
%on the current page. It can also identify the queries that uses unpredictable user input, which cannot
%be prefetched.  

We also study a specific type of query that can be prefetched: query with the same template.
An example of such query is shown in~\listref{prefetchPage}, where stories are shown by pages. 
If a user visits page 1 first (where query in~\listref{prefetchPageQ1}
is issued), and then goes to the 2nd page (where query in~\listref{prefetchPageQ2} is issued).
Since these two queries share the same format, to prefetch
the result of query in page 2 (~\listref{prefetchPageQ2}), the query plan and intermediate result
of query in~\listref{prefetchPageQ1} (for instance, the sorted {\tt stories}) can be reused.
~\figref{cacheQNumber} and~\figref{cacheQTime} show that many queries 
(40.4\% in number and 54.3\% in time) share the same template with previous queries,
revealing great opportunities in the optimization of prefetching such queries.

\begin{lstlisting}[language=Ruby,caption={Code snippet from lobsters, visiting stories listed by page}, label={prefetchPage}]
class StoriesController
  def index
    stories = Story.order('created_at').limit(40).offset(40*param[:page_id])  @\lstlabel{storyOrder}@
  end
end
\end{lstlisting}

\begin{lstlisting}[language=SQL, caption={Queries issued by Listing X, visiting page 1}, label={prefetchPageQ1}]
SELECT * from stories ORDER BY created_at LIMIT 40 OFFSET 0
\end{lstlisting}

\begin{lstlisting}[language=SQL, caption={Queries issued by Listing X, visiting page 2}, label={prefetchPageQ2}]
SELECT * from stories ORDER BY created_at LIMIT 40 OFFSET 40
\end{lstlisting}

Although most queries are prefetchable, it can be unrealistic to prefetch queries
for all possible next actions if there are many links to next pages. 
A good prediction on user behavior will help identify prefetching candidates~\cite{xxx}, 
shortening the candidate list of prefetchable actions and queries.

\begin{mybox}
\textbf{Observation}: 93.6\% of queries are prefetchable. 40.4\% of non-synthetically-equivalent
queries share the same template with previous queries. 

\textbf{Optimization}:  
\end{mybox}



==> single_query.tex <==
\section{Individual query}
In this section we study individual queries. For each potential query to be
issued in the application, we analyze how the query is issued, and how the
query result is used. 

As for how query is issued, we find that many queries (30\%) are issued in loop,
and most loops (95\%) does not have loop-carry dependency. This means that many 
prior work on query batching and set-oriented query rewriting can be applied
to most ORM applications.

As for how query result is used, we present our new findings on 
redundant data access and scalable query-result processing.
We comprehensively study how much accessed data is not used in the application,
or can be reduced by query combining. Our findings show that 
a significant portion of data (xx\%) returned is not used later in the program,
and furthermore, results of many queries (xx\%) do not need to be returned
if we can combine queries.
For scalable query-result processing, we find that many queries (xx\%) return
unbounded number of records. The result size of these queries is likely to increase
when database size increases, making the later processing on the results slow
and application unscalable. 

\subsection{Queries issued in loop}
We first analyze how query is issued, and specially focus on queries issued
in loop. These queries will be executed repeatedly with different parameters,
and are likely to become performance bottleneck. However, there are chances
to batch these queries to save roundtrip or combine them into a single query,
if loop does not have loop-carry dependency.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/general_loop.pdf}
  \caption{Queries issued in loops and whether these loops have loop-carry dependency}
  \figlabel{loop}
\vspace{-0.1in}
\end{figure}

We calculate how many queries are issued in loop, and for those loops,
how many have loop-carry dependency. In calculation, we count the query in loop
only once because it is impossible to know iteration number in static analysis.
~\figref{loop} shows that 30\% of queries are issued in loop,
and 95\% of the loops does not have loop-carry dependency. 
The result indicates that techniques presented in~\cite{xxx,xxx} can be applied
to Rails applications and have big potential for performance improvement.

\subsection{Unnecessary data retrieval}
We then analyze the data unnecessarily retrieved from the database.
Such analysis reveals the chance to improve application performance by reducing the
amount of data transferred between the application server and the database.
Our study is based on the type of such data: 
i) for each query involving single table, the columns are retrieved but not
used in the following program; ii) for each query involving multiple table (
mostly {\tt JOIN} query),
associated data retrieved but not used later; iii) the complete query results
that do not need to be returned to the program.

\paragraph{Unnecessarily retrieved columns}
A query result may contain multiple columns with some of these columns
never used by subsequent computation. We refer to these as unnecessarily
retrieved columns or redundant columns, 
which waste both computation and data transfer resources.

\tool uses static analysis to identify the columns retrieved by each query,
and then uses inter-procedural analysis to check which column is not used along 
any path from the query to the end of a controller action.
To quantify the amount of unused column data, 
we count 2450 bytes for a column with undetermined size 
(e.g., columns of type "text")\footnote{\small{~\cite{xxx} and~\cite{xxx} show the most 
popular length 
of a blog is around 2450 words and the length of a comment is around 200 words. 
We use 2450 as the default size of "text", and 200 if the field name includes "comment", 
and 128 if includes "name", "email" or "url".}} and we count the actual size
stored in the database for other columns (e.g., 4 bytes for "int"). 
The result is shown in~\figref{redundantField}.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/general_redundantField.pdf}
  \caption{Columns being retrieved but not used later in program.}
  \figlabel{redundantField}
\vspace{-0.1in}
\end{figure}


\begin{mybox}
\textbf{Observation}: More than 45\% columns retrieved in applications are not used.
%
\textbf{Optimization}: Program analysis can identify those columns, and help build
tools to rewrite queries such that only used columns are retrieved.
\end{mybox} 

Previous work has studied the unnecessary column retrieval 
problem~\cite{Chen-et-alxxx} but
has not had an effective way to automatically identify these columns, which
\tool is capable of.
Previous work \cite{Chen-et-alxxx} identifies these columns through a 
combination of static analysis and
dynamic profiling: the former analyzes ORM programs to identify 
all the used columns and dynamic 
profiling collects query logs to know which columns are retrieved. 
The reliance on dynamic profiling makes it difficult
to discover all possible redundant columns under all possible workloads. 
This limitation is addressed by \tool, which does not rely on
dynamic profiling to identify redundant columns. 
Future research can extend \tool to not only automatically
identify redundant columns, but also automatically transform the program to
eliminate unnecessary column retrieval.
 
\paragraph{Unnecessary joins}
By analyzing queries and applications, we find that
queries involving multiple tables like {\tt JOIN} query, some of the joined tables 
are not used later in the program. Some other ORM frameworks like Hibernate use eager-loading, 
where when an object retrieved, it is loaded with the associated objects 
by issuing a {\tt JOIN} query. This is likely to cause unnecessary join problem
when the associated objects are not used later in the program (studied in~\cite{xxx}).
Different from these frameworks, Rails uses lazy loading, where only the object is loaded.
However, since the lazy loading scheme may cause ``N+1'' problem~\cite{xxx}, 
developers are encouraged to use functions like {\tt includes} to specify associated
objects to be eager-loaded. As an example shown in~\listref{unusedJoin}, when a {\tt todo}
object is loaded, a query shown in~\listref{unusedJoinQuery} is issued 
to preload all associated projects,
tags, and predecessor todo.

\begin{lstlisting}[language=Ruby,caption={Code snippet from tracks, 
example of unnecessary join with lazy loading},label={unusedJoin}]
def load_todo(condition)
  return Todo.where(condition).includes(:projects, :tags, :predecessor) @\lstlabel{loadTodo}@
end
def show_recent_todos
  todos = load_todo('created_at > #{Time.now-10.days}')
  pred = todos.predecessors  @\lstlabel{useTodo}@
end
\end{lstlisting}

\begin{lstlisting}[language=SQL,caption={Query issued by code in Listing X},label={unusedJoinQuery}]
SELECT * from todos AS t1 WHERE created_at > '2016-11-01' INNER JOIN projects AS p ON p.id = t1.project_id INNER JOIN tags AS t ON t.id = t1.tag_id INNER JOIN todos AS t2 ON t1.predecessor_id = t2.project_id
\end{lstlisting}

Even for ORM using lazy-loading scheme, unnecessary join problem may also occur
due to program practice. In~\listref{unusedJoin}, among the other objects eager-loaded with
the {\tt todo} object, only the predecessor todo is used in the program 
as shown on~\lstref{useTodo}, leaving the other joined tables unused.
We analyze how frequently such unnecessary join happens among all join queries loading
associated objects,
and the result is shown in~\figref{redundantTable}.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/general_redundantTable.pdf}
  \caption{For all join queries loading associate data, the number of joins whose data is being used/not used in the program}
  \figlabel{redundantTable}
\vspace{-0.1in}
\end{figure}

\begin{mybox}
\textbf{Observation}: 31\% of the joins involved in {\tt JOIN} queries loading associated
data is not necessary in the program, even when all eager-loaded objects are specified
by programmer.
%
\textbf{Optimization}: Program analysis can identify associated objects used in the program.
and tool using such analysis is able to automatically eager-load only needed associated objects.
\end{mybox}

\paragraph{Unnecessary queries}
We also look into unnecessary data retrieval at query level.
 If the result returned by a query {\tt Q} is only used as parameters to other queries {\tt Q1, Q2...}, 
combining {\tt Q} with {\tt Q1, Q2...} into join queries or stored procedures can avoid returning
the results from {\tt Q} to application.
We count the number of such queries whose result is only used for other queries, 
and the result is shown in~\figref{queryOnlyToQuery}.

%The performance benefit is significant when the number tuples returned by {\tt Q} is 
%large and the network delay between the database and application server is non-negligible.
The performance benefit of combing queries to avoid unnecessary data return is significant
when the number tuples returned by {\tt Q} is large.
~\listref{issueSelect} shows an example. The action shows all issues
belonged to members belonging to group 1. Query on~\lstref{select1} 
in the original implementation returns all members from group 1, the result of which
is only used for query on~\lstref{select2}. These two queries can be combined into a single
query as shown in~\listref{issueJoin}. 
We tested the performance gain of query combining, with database configurations
in which the query on~\lstref{select1} returns xxK records.
The query execution time under different network delay
configuration is listed in~\tableref{networkDelayEffect}.
%, which shows that combining queries shows greater
%benefit when the network delay increases.

\begin{lstlisting}[language=SQL, caption={Queries retrieving issues created by members belong to group 1.
Code abridged from redmine.}, label={issueSelect}]
Q1: SELECT * FROM members WHERE group_id = 1;  @\lstlabel{select1}@
Q2: SELECT * FROM issues WHERE creator_id IN (...) AND AND is_public = 1 @\lstlabel{select2}@
\end{lstlisting}

\begin{lstlisting}[language=SQL, caption={Combining Q1 and Q2 in Listing X}, label={issueJoin}]
SELECT * FROM issues INNER JOIN members ON members.group_id = 1 AND issues.creator_id = members.id AND issues.is_public = 1 
\end{lstlisting}

\cong{Smaller network delay result TBD.}
%
\begin{table}[]
\centering
\caption{Evaluation on the reduction in query time of query combining. Q1 returns 20K records, with each record 17 bytes.}
\label{networkDelayEffect}
\begin{tabular}{lllll}
network\_delay & Q1   & Q2   & JoinQ & Reduced     \\
10ms           & 0.85 & 0.25 & 0.19  & 0.827272727 \\
100ms          & 1.04 & 1.3  & 1.24  & 0.47008547  \\
1000ms         & 12   & 14.8 & 8.05  & 0.699626866
\end{tabular}
\end{table}


\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/general_queryOnlyToQuery.pdf}
  \caption{Queries whose result is only used in other queries.}
  \figlabel{queryOnlyToQuery}
\vspace{-0.1in}
\end{figure}


\begin{mybox}
\textbf{Observation}: 29\% of read queries return results that are only
 used to issue other queires.

\textbf{Optimization}: Program analysis is able to identify such queries, 
and it can help build tools to combine such queries into other queries
to reduce the data transfered between application server and database.
\end{mybox}

\subsection{Scalable query-result processing}
Developers usually wish their application to be scalable with larger data, 
meaning that the response time does not increase significantly when the size of 
database increases. We briefly break the response time into the time spent on 
database and on application server.

Armbrust et al.~\cite{xxx} discussed about the scalability of queries,
and how to convert scale-dependent queries into scale-independent 
queries, so we emit our discussion on the time spent on the database.
We focus on the scalability of the time spent on the server, which mainly
includes the time spent in controller to process query results, and in view
to render the results.

Intuitively, when database size increases, some queries return larger number
of records, which makes the later processing slower. We look into the relationship
between the number of returned records and the server time. In profiling, 
and count the total number of records returned by database in an action
and check the time spent on the server of that action. The result 
in~\figref{resultsizeTime} show that if a query returns large number of records,
the afterwards processing on server is likely to be slow\footnote{\small{We manually check
the dots on the right bottom of~\figref{resultsizeTime}, where a lot of records
are returned but server running time is small, and we find that these actions are
issueing unnecessary queries which can be combined into other queries, as discussed
in section x.}}, while if all queries return small number of records, the the server
processing is fast.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/resultsize_time.pdf}
  \caption{The relationship between the total number of records and the server running
time. Each point represents a single response (server action). For each application,
the x-axis value of a point $i$ is
${{{\rm{\# records\_in\_actio}}{{\rm{n}}_i}} \over {\max ({\rm{\# records\_in\_actio}}{{\rm{n}}_{k,k \in [1,...,n]}})}}$
(fraction to the max number of records returned to an action),
and y-axis value is 
${{{\rm{server\_time\_of\_actio}}{{\rm{n}}_i}} \over {\max ({\rm{server\_time\_of\_actio}}{{\rm{n}}_{k,k \in [1,...,n]}})}}$
(fraction to the max server running time of an action).
The max value of each application is as follow: a. gitlab (100K records, 36sec); b. kandan (150K, 8sec);
c. lobsters (100K, 11sec); d. redmine (140K, 311sec); e. sugar (150K, 22sec); f. tracks (90K, 111sec).
}
\figlabel{resultsizeTime}
\vspace{-0.1in}
\end{figure}


%Since the applications running time varies due to the loops, we study the
%loops and check what affects the loop iteration. In all applications we studied, more than
%98\% of loops are iterating over an array or hash table (while the rest 2\% 
%has iterations dependent
%on specific variable value), and more than 49\% of the loops
%are one-by-one processing the results.
%When database size increases, half of the loops may becomes
%slower since the query may return more records, thus increasing the loop iteration
%and making the response slow.

%We then study the size of query results. If a query returns a large result set, 
%subsequent computation processing the results takes a long time to complete. 
%Queries whose result set size increases with the database size are 
%important causes for applications's scalability problem.
%
%\cong{How to make this more clear? Is it important?}
%We first look into the relationship between the query result size and the application's
%scalability. Since the applications running time varies due to the loops, we study the
%loops and check what affects the loop iteration. In all applications we studied, more than
%98\% of loops are iterating over an array or hash table (while the rest 2\% 
%has iterations dependent
%on specific variable value), and more than 49\% of the loops
%are one-by-one processing the results.
%%(while other array-iterating loops are processing
%%user inputs, or other data).
%The above finding shows that when database size increases, half of the loops may becomes
%slower since the query may return more records, thus increasing the loop iteration.
%%, while
%%the values of records in database trivially matters since they affect less than 2\% of 
%%loops in application.

Based on the above finding, we then analyze the number of records returned by each query.
In Rails, if a query always returns a single value (e.g., a COUNT query), 
a single record (e.g., retrieving using a unique identifier), 
or has a LIMIT keyword, the number of returned records of that query is bounded, 
otherwise the query result sizes is unbounded and hence likely scale with the database size.
The result of read query breakdown into queries returning bounded/unbounded 
results are shown in~\figref{queryCard}.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth]{figs/general_queryCard.pdf}
  \caption{Queries returning bounded/unbounded numbers of records}
  \figlabel{queryCard}
\vspace{-0.1in}
\end{figure}

Restricting the number of returned records helps improve application's scalability,
but requires corresponding changes in the application code. For instance, if an application
designer wishes to show all the comments on a single webpage, an alternative way of
retrieving all comments and rendering them, which makes the response time increase linearly
with the {\tt Comment} table size, is to render some of the comments when the webpage
returns, and incrementally loading other comments when the user scrolls down the page. 
We manually changed the application code to implement such incremental loading mechanism,
restricting the number of records returned by each query issued when generating the response
for certain requests. The results presented in~\figref{pageScroll} shows great performance improvement
(xx\% reduction in initial response time). 

\cong{Showing the total time of initial page loading + all scrolls? TBD}
\begin{figure}[h]
  \centering
  \includegraphics[page=1, width=1\columnwidth]{figs/test-crop.pdf}
  \caption{Performance improvement of incremental data loading. On the left shows the 
Activity.index action from redmine application, with 20K records rendered on a single page. 
On the right shows Todos.index action from tracks, with 20K records on one page. 
For each subfigure, the left most bar shows the original page response time; 
the middle bar shows the response time of the initial page showing only the first 40 records; 
the right most bar shows the time it takes on each scroll, 
which append another 40 records to the page. }
  \figlabel{pageScroll}
\vspace{-0.1in}
\end{figure}

From above, our study shows that program analysis can help identify the queries
returning unbounded results
After recognizing those queries, a tool
can be built to change such queries to return bounded records, and 
automatically adapt the application code to implement incremental loading.

\begin{mybox}
\textbf{Observation}: A non-trivial number of queries (35\%) return unbounded result sets.

\textbf{Optimization}: Sucn queries make application vulnerable to scalability problems, and
program analysis
can help identify such queries.
\end{mybox}


